Lingjing: A Simulation Testbed for Multi-Agent Embodied Tasks in Open-Ended Cities

Urban embodied intelligence requires coordination among heterogeneous agents (e.g., UAVs, ground robots, and autonomous vehicles) in dynamic cities. Simulators therefore provide a scalable foundation for developing and evaluating such coordination. Existing platforms nevertheless isolate different embodiments and decouple them from task design and evaluation. We present \textbf{Lingjing}, a simulation platform for heterogeneous multi-agent embodied intelligence in open-ended urban environments. Lingjing reconstructs and renders evolving cities from geographic data, synchronizes multiple physics engines, and exposes shared physical and structured urban state to agents. Its Gym-like interface supports user-defined ReAct agents and single- or multi-agent natural-language missions with configurable star or broadcast communication and resource constraints. Each episode becomes an attribution-ready replay that links agent trajectories and communication to relation-graph changes, resource consumption, and engine-based evaluations for systematic diagnosis. We evaluate twelve vision-language models on nine urban tasks under a shared engine-in-the-loop protocol. Controlled studies further examine communication, scalability, robustness, and failure provenance. Results expose persistent bottlenecks in grounding and long-horizon execution. They also show task-dependent coordination trade-offs and diminishing returns from added capacity, while heavier workloads further reduce success. Lingjing provides a unified testbed that enables reproducible end-to-end evaluation and systematic failure diagnosis in urban multi-agent embodied intelligence.

==> sections/00_abstract.tex <==
\begin{abstract}
Urban embodied intelligence requires heterogeneous agents---such as UAVs, ground robots, autonomous vehicles, and fixed infrastructure---to coordinate over dynamic cities, yet existing simulators typically isolate embodiments, tasks, or evaluation signals. We present Lingjing, a simulation platform for heterogeneous multi-agent embodied intelligence in open-ended urban environments. Lingjing reconstructs evolving cities from geographic data, synchronizes multiple physics engines, and exposes shared physical and structured urban state to agents. Its Gym-like interface supports user-defined ReAct agents and natural-language missions at individual, group, and system levels, with configurable communication and resource constraints. Each episode is recorded as a replayable, attribution-oriented artifact containing observations, actions, inter-agent messages, relation-graph updates, token and cost traces, and engine-based evaluation signals, enabling diagnostic analysis and causal interventions. We evaluate nine urban tasks with twelve vision-language backbones under controlled engine-in-the-loop protocols, including star and broadcast coordination. The results show that scaling improves aggregate success but not uniformly across tasks, topology benefits depend on the coordination bottleneck, photorealistic appearance affects small-target detection, and explicit prompt structure improves executable actions. Lingjing provides a unified and reproducible testbed that measures end-to-end performance while localizing perception, localization, handoff, coordination, and long-horizon execution failures.
\end{abstract}
% Multimodal large language models and the Vision--Language--Action (VLA)
% policies built on top of them are quickly becoming the foundation of embodied
% AI, and the most consequential places to deploy them are \emph{future cities}:
% last-mile delivery, infrastructure inspection, emergency response, fleet
% logistics, and 24/7 urban services all hinge on heterogeneous robots, UAVs,
% and vehicles coordinating across blocks. Training and evaluating such agents
% directly in real cities, however, is prohibitively expensive, unsafe at scale,
% hard to reproduce, and impossible to rewind, which makes simulation the only
% path that scales without giving up scientific control. Yet the simulators most
% embodied-agent benchmarks build on still focus on a single domain---indoor
% navigation, tabletop manipulation, or solo autonomous driving---and rarely
% capture dynamic urban environments where heterogeneous embodied agents must
% coordinate over long horizons under traffic, weather, occlusion,
% communication limits, and shifting priorities.
% % 中文翻译：
% % 多模态大语言模型及其之上的视觉--语言--动作（VLA）策略正迅速成为具身智能的基础，而最有影响力的部署场景是未来城市：
% % 末端配送、基础设施巡检、应急响应、车队物流和全天候城市服务都依赖异构机器人、无人机和车辆跨街区协同。
% % 然而，直接在真实城市中训练和评估这类智能体成本极高、规模化不安全、难以复现且无法回放，因此仿真是在不牺牲科学控制的前提下实现规模化的唯一路径。
% % 可是，大多数具身智能基准所依赖的仿真器仍聚焦于单一领域，例如室内导航、桌面操作或单车自动驾驶，
% % 很少刻画异构具身智能体必须在交通、天气、遮挡、通信限制和动态优先级下进行长时程协同的城市环境。

% We present \textbf{Lingjing}, a simulation platform whose three pillars are
% (i) a dynamic urban environment that exposes both pixel-level and structured
% city state; (ii) a System--Group--Individual hierarchical VLA interface that
% lets heterogeneous embodied agents be coordinated through natural-language
% missions; and (iii) a real-time WebSocket bridge to an Unreal-Engine renderer
% paired with a trajectory recorder that turns every episode into replayable
% task evidence. Built on this substrate, \textbf{Lingjing-Bench} defines nine
% representative runnable tasks spanning single-agent grounding, multi-agent
% coordination, and system-level replanning. Its evaluation protocol compares
% commercial and open-source model backbones and goes beyond success rate by
% measuring communication cost, sub-task provenance, dependency violations,
% loop/deadlock events, and per-category failure attribution. Lingjing therefore
% supports studying urban embodied intelligence as a coordination problem under
% realistic dynamics, rather than as a sequence of isolated single-agent tasks.
% % 中文翻译：
% % 我们提出 \textbf{Lingjing}，这是一个由三大支柱构成的仿真平台：（i）同时暴露像素级与结构化城市状态的动态城市环境；
% % （ii）通过自然语言任务协调异构具身智能体的 System--Group--Individual 分层VLA 接口；
% % （iii）连接 Unreal Engine 渲染器的实时 WebSocket 桥接器，以及将每个 episode 转化为可回放任务证据的轨迹记录器。
% % 在这一基础上，\textbf{Lingjing-Bench} 定义了九个具有代表性的可运行任务，覆盖单智能体 grounding、多智能体协同和系统级重规划。
% % 其评估协议比较商业与开源模型骨干，并超越成功率，进一步度量通信成本、子任务来源、依赖违例、循环/死锁事件和分类失败归因。
% % 因此，Lingjing 支持将城市具身智能作为真实动态下的协同问题来研究，而不是把它视作一串孤立的单智能体任务。



==> sections/05_experiments_copy.tex <==
\section{Experiments}
\label{sec:experiments}
\begin{table*}[ht]
	\centering
	\begin{minipage}[t]{0.7\textwidth}
		\vspace{0pt}
		\centering\scriptsize
		\setlength{\tabcolsep}{2.6pt}
		\resizebox{0.9\linewidth}{!}{%
			\begin{tabular}{@{}l*{13}{c}@{}}
				\toprule
				\textbf{Backbone} & VDN & BI & LD & IDF & UPR & UFR$^{s}$ & UFR$^{b}$ & CR & SSR$^{s}$ & SSR$^{b}$ & CD$^{s}$ & CD$^{b}$ & Avg \\
				\midrule
				\multicolumn{14}{@{}l}{\new{\emph{Commercial models}}} \\
				GPT-5.5~\cite{gpt55}         & \new{\textbf{72}} & \new{\textbf{40}} & \new{\underline{48}} & \new{79} & \new{\underline{47}} & \new{\textbf{63}} & \new{\underline{67}} & \new{\underline{74}} & \new{\underline{79}} & \new{\underline{84}} & \new{\textbf{90}} & \new{\textbf{78}} & \new{\textbf{66}} \\
				GPT-5.4~\cite{gpt54}         & \new{\underline{66}} & \new{34} & \new{43} & \new{\textbf{86}} & \new{42} & \new{58} & \new{64} & \new{\textbf{80}} & \new{75} & \new{82} & \new{\underline{86}} & \new{\underline{74}} & \new{63} \\
				Gemini-3.1-Pro~\cite{gemini31pro}  & \new{64} & \new{\underline{37}} & \new{\textbf{52}} & \new{\underline{81}} & \new{44} & \new{\underline{61}} & \new{\textbf{70}} & \new{69} & \new{\textbf{83}} & \new{\textbf{87}} & \new{80} & \new{69} & \new{\underline{64}} \\
				Kimi-K2.5~\cite{kimik25}       & \new{51} & \new{23} & \new{36} & \new{54} & \new{28} & \new{47} & \new{41} & \new{61} & \new{46} & \new{58} & \new{60} & \new{45} & \new{45} \\
				Qwen3-VL-Flash~\cite{qwen3vlflash}  & \new{39} & \new{25} & \new{31} & \new{46} & \new{\textbf{50}} & \new{38} & \new{47} & \new{52} & \new{49} & \new{55} & \new{51} & \new{44} & \new{43} \\
				\midrule
				\multicolumn{14}{@{}l}{\new{\emph{Open-source models}}} \\
				Qwen3-VL-2B~\cite{qwen3vl}     & \new{38} & \new{16} & \new{27} & \new{29} & \new{18} & \new{30} & \new{27} & \new{46} & \new{35} & \new{33} & \new{34} & \new{36} & \new{30} \\
				Qwen3-VL-4B~\cite{qwen3vl}     & \new{44} & \new{24} & \new{25} & \new{38} & \new{26} & \new{33} & \new{41} & \new{45} & \new{40} & \new{44} & \new{47} & \new{35} & \new{36} \\
				Qwen3-VL-8B~\cite{qwen3vl}     & \new{48} & \new{31} & \new{37} & \new{49} & \new{29} & \new{46} & \new{50} & \new{56} & \new{45} & \new{59} & \new{55} & \new{48} & \new{45} \\
				InternVL3.5-8B~\cite{internvl35}  & \new{43} & \new{28} & \new{30} & \new{47} & \new{23} & \new{41} & \new{36} & \new{53} & \new{44} & \new{47} & \new{52} & \new{39} & \new{39} \\
				Pixtral-12B~\cite{pixtral12b}     & \new{52} & \new{21} & \new{35} & \new{40} & \new{27} & \new{34} & \new{40} & \new{47} & \new{38} & \new{50} & \new{46} & \new{42} & \new{39} \\
				MiniCPM-V-4.5~\cite{minicpmv45}   & \new{34} & \new{22} & \new{21} & \new{33} & \new{20} & \new{32} & \new{29} & \new{39} & \new{34} & \new{32} & \new{40} & \new{31} & \new{30} \\
				Gemma-3-4B~\cite{gemma3}      & \new{30} & \new{17} & \new{23} & \new{26} & \new{16} & \new{25} & \new{31} & \new{42} & \new{29} & \new{35} & \new{32} & \new{27} & \new{27} \\
				\bottomrule
			\end{tabular}
		}
		\caption{Engine-adjudicated TSR (\%) on nine tasks. Superscripts $s$ and $b$ denote star and broadcast. Avg averages modes within UFR, SSR, and CD before the nine-task mean. Bold and underlined values are the best and second-best.}
		\label{tab:main}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{0.24\textwidth}
		\vspace{0pt}
		\centering\scriptsize
		\renewcommand{\arraystretch}{0.74}
		\setlength{\tabcolsep}{2pt}
		\resizebox{0.9\linewidth}{!}{%
			\begin{tabular}{@{}llrr@{}}
				\toprule
				\textbf{Task} & \textbf{Metric} & \textbf{Star} & \textbf{Broad.} \\
				\midrule
				CD  & TSR (\%)              & \textbf{62}  & 48 \\
				& Messages              & \textbf{6}   & 38 \\
				& Payload (KB)          & \textbf{0.7} & 1.9 \\
				& Rounds                & \textbf{4}   & 12 \\
				& Assignment gap (\%)   & \textbf{10}  & 22 \\
				& Repeated target (\%)  & \textbf{14}  & 20 \\
				\midrule
				UFR & TSR (\%)              & 55           & \textbf{60} \\
				& Messages              & \textbf{6}   & 61 \\
				& Payload (KB)          & \textbf{0.5} & 3.0 \\
				& Rounds                & \textbf{5}   & 9 \\
				& Assignment gap (\%)   & \textbf{13}  & 15 \\
				& Repeated target (\%)  & 17           & \textbf{11} \\
				\midrule
				SSR & TSR (\%)              & 58           & \textbf{74} \\
				& Messages              & \textbf{5}   & 9 \\
				& Payload (KB)          & \textbf{0.4} & 0.7 \\
				& Rounds                & \textbf{5}   & 8 \\
				& Assignment gap (\%)   & 16           & \textbf{11} \\
				& Repeated target (\%)  & 23           & \textbf{9} \\
				\bottomrule
			\end{tabular}
		}
		\caption{Communication modes on matched instances with fixed qwen3.7-plus. Bold marks the better value.}
		\label{tab:comm}
	\end{minipage}
\vspace{-0.5cm}
\end{table*}
\subsection{Experimental Setup}
\label{sec:exp:setup}

\textbf{Backbones.} We evaluate twelve multimodal backbones in one scaffold: five commercial models (GPT-5.5~\cite{gpt55}, GPT-5.4~\cite{gpt54}, Gemini-3.1-Pro~\cite{gemini31pro}, Kimi-K2.5~\cite{kimik25}, and Qwen3-VL-Flash~\cite{qwen3vlflash}) and seven open-weight models (Qwen3-VL-2B/4B/8B~\cite{qwen3vl}, InternVL3.5-8B~\cite{internvl35}, MiniCPM-V-4.5~\cite{minicpmv45}, Gemma-3-4B~\cite{gemma3}, and Pixtral-12B~\cite{pixtral12b}). Per task, all share observation encoding, prompt, action schema, and communication interface without specific fine-tuning. Superscripts $s$ and $b$ denote star and broadcast. Each diagnostic states its backbone, while scaffold analyses use qwen3.7-plus~\cite{qwen37plus} to balance performance and cost.

\textbf{Metrics.} Task success rate (TSR) is the percentage of episodes satisfying all engine-adjudicated terminal conditions within budget. Adjudication uses engine proximity and events, not model self-reports, with geometry- and motion-based acceptance regions fixed across backbones and communication modes. Intermediate detections only unlock later stages. Avg is the unweighted mean TSR across tasks, and subtask completion rate (SCR) measures partial progress in multi-target or multi-stage missions. Other metrics are defined at first use. Appendices~\ref{app:adjudication} and~\ref{app:metrics} give all task conditions and definitions.

\textbf{Implementation Details.} Open-source models use vLLM in bfloat16 with a 16K context on four NVIDIA A800 GPUs, while commercial models use provider endpoints. Within each task, all models share the prompt and $2048$-token output limit, use provider-specific near-greedy decoding, and perform both visual analysis and action selection. Unless stated otherwise, each model and diagnostic condition uses $100$ matched seeded instances from fixed templates and initial poses, with seeds also controlling entity subsets, while larger-sample studies report their sizes explicitly. Agents receive visual and structured observations, history, messages, and coarse search regions but not hidden-target coordinates, then emit physical actions and optional messages. Fixed time and step budgets bound each episode. Vision timeouts count as no detections, while infrastructure failures are tracked separately. Additional communication, intervention, appearance, component, and prompt analyses appear in Appendices~\ref{app:bench} and~\ref{app:lastmile}.

\subsection{Main Results}
\label{sec:exp:main}

Table~\ref{tab:main} shows GPT-5.5 leading with an Avg of $66$, followed by Gemini-3.1-Pro at $64$ and GPT-5.4 at $63$. Across the twelve task-mode columns, GPT-5.5 leads five, Gemini-3.1-Pro four, GPT-5.4 two, and Qwen3-VL-Flash one. Qwen3-VL-8B is the strongest open-source model at $45$, tying Kimi-K2.5 and exceeding its 2B and 4B variants by $15$ and $9$ points, although task-level scaling is not monotonic. BI, UPR, and LD remain hardest, with best TSRs of $40$, $50$, and $52$, exposing bottlenecks in localization, constrained planning, and multi-stage execution beyond visual recognition. Broadcast outperforms star for $8/12$ UFR and $10/12$ SSR backbones, whereas star wins $11/12$ CD comparisons. Routing gains therefore depend on task structure rather than message reach alone. Section~\ref{sec:exp:comm} analyzes the associated communication cost.

\subsection{Communication Modes and Cost}
\label{sec:exp:comm}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{photo/logistic_1.pdf}
%	\caption{\new{Representative city-logistics traces with fixed qwen3.7-plus. Star splits the $250$\,kg order \texttt{del-001}, whereas broadcast leaves it unassigned.}}
%	\label{fig:logistics-traces}
%\end{figure}
%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{photo/logistic_2.pdf}
%	\caption{\new{Matched-instance city-logistics outcomes with fixed qwen3.7-plus. Star increases TSR and reduces all reported coordination measures.}}
%	\label{fig:logistics-outcomes}
%\end{figure}
\begin{figure}[t]
	\centering
	\begin{minipage}[t]{0.8\linewidth}
		\centering
		\includegraphics[width=\linewidth]{photo/logistic_1.pdf}
		\\[-0.4em]\footnotesize (a)
	\end{minipage}
	\hfill
	\begin{minipage}[t]{0.8\linewidth}
		\centering
		\includegraphics[width=\linewidth]{photo/logistic_2.pdf}
		\\[-0.4em]\footnotesize (b)
	\end{minipage}
	\caption{\new{City-logistics comparison with fixed qwen3.7-plus. (a) Representative traces, where star splits the $250$\,kg order \texttt{del-001} and broadcast leaves it unassigned. (b) Matched-instance outcomes, where star increases TSR and reduces all reported coordination measures.}}
	\label{fig:logistics-process}
\end{figure}

With qwen3.7-plus and matched instances fixed, only routing varies: star uses a coordinator, whereas broadcast reaches all peers (Table~\ref{tab:comm}). In CD (Figs.~\ref{fig:logistics-traces} and~\ref{fig:logistics-outcomes}), star splits the $250$\,kg order while broadcast leaves it unassigned, raising TSR from $48$ to $62$ while cutting messages from $38$ to $6$ and the assignment gap from $22\%$ to $10\%$. Supplementary sea-rescue traces and matched-instance results appear in the appendix (Fig.~\ref{fig:sea-process}). UFR shows a weaker trade-off: broadcast adds five TSR points but increases messages from $6$ to $61$. Thus, star favors structured allocation, whereas broadcast benefits rapid discovery sharing at higher communication cost.

\subsection{Subtask Provenance}
\label{sec:exp:subtask}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{photo/subtask_provenance.pdf}
    \caption{\new{Subtask provenance and perception diagnosis. (a) Cumulative stage success reveals where errors enter and propagate from detection to engine-adjudicated execution. (b) $1-\mathrm{F1}$, miss rate, normalized LocErr, and ECE distinguish detection, localization, and calibration errors, with higher values indicating worse performance.}}
    \label{fig:subtask-provenance}
\end{figure}
    
Using fixed qwen3.7-plus over $100$ episodes per mission, we reconstruct cumulative provenance chains for UAV-guided pipeline repair (UPR), UAV--fire-truck response (UFR), and sea search and rescue (SSR). A stage succeeds only if all preceding stages also succeed, allowing panel (a) to locate stage-wise attrition and panel (b) to relate it to detection, localization, or calibration errors. F1 is the harmonic mean of frame-level precision and recall, while miss rate is the share of all aligned frames containing a missed target. LocErr is the median world-coordinate error of matched true positives, normalized by the largest mission value in panel (b). Expected calibration error (ECE) is the ten-bin weighted gap between confidence and observed accuracy. Figure~\ref{fig:subtask-provenance} identifies detection-to-location grounding as the largest loss: $28$, $19$, and $14$ points for UPR, UFR, and SSR, versus subsequent losses of $15$, $11$, and $8$ points. Despite per-frame miss rates of $74\%$ for UPR and $71\%$ for SSR, repeated observations raise cumulative detection to $88\%$ and $96\%$. UFR achieves the best F1 ($0.76$) and ECE ($0.08$), while UPR has the worst ECE ($0.69$) and SSR the largest LocErr ($190$\,m). Thus, repeated sensing improves coverage but not necessarily grounded handoffs. Appendix~\ref{app:lastmile} further analyzes staged error interventions for the last-mile delivery task.


\subsection{Scaling and Robustness}
\label{sec:exp:scaling}

\begin{figure}[ht]
	\centering
	\begin{minipage}[t]{0.8\linewidth}
		\vspace{0pt}
		\centering
		\includegraphics[width=\linewidth]{photo/scaling_sweeps.pdf}
		\\[-0.4em]\footnotesize Top
	\end{minipage}
	\vspace{0.4em}
	\begin{minipage}[t]{0.8\linewidth}
		\vspace{0pt}
		\centering
		\includegraphics[width=\linewidth]{photo/robustness_sweeps.pdf}
		\\[-0.4em]\footnotesize Bottom
	\end{minipage}
	\caption{Scaling and robustness analyses. Top: team-size and workload sweeps over SSR UAV count, UFR fire count, and CD delivery-point count. Bottom: robustness sweeps over SSR sensing settings and LD, CR, and UPR control budgets.}
	\label{fig:scale-robust}
\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{photo/scaling_sweeps.pdf}
%    \caption{Team-size and workload sweeps. (a) SSR UAV count. (b) UFR fire count. (c) CD delivery-point count.}
%    \label{fig:scale}
%\end{figure}
Scaling uses GPT-5.5 and Qwen3-VL-8B with $100$ matched episodes per point. Under broadcast, SSR sweeps UAVs from $1$ to $3$ with three victims, UFR fires from $2$ to $6$ with five UAVs, and CD under star delivery points from $5$ to $20$ with five vehicles. Shared seeds select targets and recompute ground truth and terminal criteria. Figure~\ref{fig:scale} shows diminishing capacity returns and workload degradation. Adding a second SSR UAV raises TSR by $19/17$ points and a third by $9/11$ for GPT-5.5/Qwen3-VL-8B. From lowest to highest workload, UFR falls by $20/19$ points and CD by $7/19$. GPT-5.5 leads throughout, while Qwen3-VL-8B is more sensitive to CD load.

%\begin{figure}[!htbp]
%    \centering
%    \includegraphics[width=\linewidth]{photo/robustness_sweeps.pdf}
%    \caption{Robustness sweeps. (a) SSR altitude, coverage, and LocErr. (b) SSR grid-resolution and overlap sweeps. (c) Maximum LD dog moves, CR vehicle replans, and UPR guidance steps.}
%    \label{fig:robust}
%\end{figure}

Fixing qwen3.7-plus, we run $200$ matched episodes per point to reduce variance and sweep SSR altitude ($60/100/140$\,m), grid resolution ($2\!\times\!2/3\!\times\!3/4\!\times\!4$), overlap ($0.1/0.2/0.4$), and control budgets for LD moves ($25/50/75$), CR replans ($0/3/6$), and UPR guidance ($10/20/30$). Success is cumulative S4 legal-edge arrival for LD and engine-adjudicated destination arrival or leak sealing for CR/UPR, with other settings fixed. Figure~\ref{fig:robust} shows a coverage-precision trade-off and diminishing budget returns. Altitude $60\to140$\,m raises coverage $64\%\to90\%$ but LocErr $112\to286$\,m. Grid and overlap yield coverage $63\%\to82\%\to91\%$ and $74\%\to82\%\to89\%$, respectively. Tight-to-default budgets add $8.0/29/12$ points for LD/CR/UPR, versus $5.5/2/4.5$ from default-to-loose. Defaults capture most available gains.

